Boosting the Capabilities of Compact Models in Low-Data Contexts with Large Language Models and Retrieval-Augmented Generation

The data and compute requirements of current language modeling technology pose challenges for the processing and analysis of low-resource languages. Declarative linguistic knowledge has the potential to partially bridge this data scarcity gap by providing models with useful inductive bias in the form of language-specific rules. In this paper, we propose a retrieval augmented generation (RAG) framework backed by a large language model (LLM) to correct the output of a smaller model for the linguistic task of morphological glossing. We leverage linguistic information to make up for the lack of data and trainable parameters, while allowing for inputs from written descriptive grammars interpreted and distilled through an LLM. The results demonstrate that significant leaps in performance and efficiency are possible with the right combination of: a) linguistic inputs in the form of grammars, b) the interpretive power of LLMs, and c) the trainability of smaller token classification networks. We show that a compact, RAG-supported model is highly effective in data-scarce settings, achieving a new state-of-the-art for this task and our target languages. Our work also offers documentary linguists a more reliable and more usable tool for morphological glossing by providing well-reasoned explanations and confidence scores for each output.

==> tables/old_baseRAG.tex <==
\begin{table*}[h!]
    \centering
    \renewcommand{\arraystretch}{1.5} % Provides more space between rows for better readability
    \begin{tabular}{|c|c|c|c|c|} \hline
        Model & \multicolumn{2}{c|}{Uspanteko} & \multicolumn{2}{c|}{Arapaho} \\ \cline{2-5}
              & Word-level & Morpheme-level & Word-level & Morpheme-level \\
              & Accuracy & Accuracy & Accuracy & Accuracy \\ \hline
        RoBERTa Baseline & 76.55 & 82.48 & 85.44 & 91.11 \\ \hline
        Bi-LSTM Baseline & 71.28 & 73.90 & 76.41 & 80.44 \\ \hline
        GPT-4 Baseline (Zero-shot RAG) & 42.21 & 51.88 & 48.47 & 53.48 \\ \hline
        Claude Baseline (Zero-shot RAG) & 38.40 & 42.21 & 49.91 & 58.60 \\ \hline
        RoBERTa + Claude (Train + RAG) & \textbf{79.21} & \textbf{84.84} & \textbf{86.82} &\textbf{ 93.74} \\ \hline
        RoBERTa + GPT-4 (Train + RAG) & 78.41 & 81.49 & 85.51 & 91.43 \\ \hline
        Bi-LSTM + Claude (Train + RAG) & 77.47 & 80.21 & 79.12 & 85.44 \\ \hline
        Bi-LSTM + GPT-4 (Train + RAG) & 73.17 & 78.23 & 74.16 & 81.31 \\ \hline
    \end{tabular}
    \caption{Comparison of model performances on word-level and morpheme-level accuracy for Uspanteko and Arapaho languages}
    \label{tab:naive_rag}
\end{table*}

==> tables/old_modRAG.tex <==

\begin{table*}[h!]
    \centering
    \renewcommand{\arraystretch}{1.5} % Provides more space between rows for better readability
    \begin{tabular}{|c|c|c|c|c|} \hline
        \multirow{2}{*}{Model} & \multicolumn{2}{c|}{Uspanteko} & \multicolumn{2}{c|}{Arapaho} \\ \cline{2-5}
                               & Word-level & Morpheme-level & Word-level & Morpheme-level \\
                               & Accuracy & Accuracy & Accuracy & Accuracy \\ \hline
        RoBERTa + Claude & 81.12 & 85.02 & 83.48 & 91.26 \\ \hline
        RoBERTa + GPT-4 & 79.44 & 82.98 & 82.41 & 88.68 \\ \hline
        Bi-LSTM + Claude & 78.26 & 82.22 & 81.24 & 85.89 \\ \hline
        Bi-LSTM + GPT-4 & 74.12 & 78.99 & 76.77 & 82.18 \\ \hline
    \end{tabular}
    \caption{Modular RAG applied to Uspanteko and Arapaho Languages with RoBERTa and Bi-LSTM training}
    \label{tab:modular_rag}
\end{table*}
